Augmented Bilinear Network for Incremental Multi-Stock Time-Series Classification

Deep Learning models have become dominant in tackling financial time-series analysis problems, overturning conventional machine learning and statistical methods. Most often, a model trained for one market or security cannot be directly applied to another market or security due to differences inherent in the market conditions. In addition, as the market evolves through time, it is necessary to update the existing models or train new ones when new data is made available. This scenario, which is inherent in most financial forecasting applications, naturally raises the following research question: How to efficiently adapt a pre-trained model to a new set of data while retaining performance on the old data, especially when the old data is not accessible? In this paper, we propose a method to efficiently retain the knowledge available in a neural network pre-trained on a set of securities and adapt it to achieve high performance in new ones. In our method, the prior knowledge encoded in a pre-trained neural network is maintained by keeping existing connections fixed, and this knowledge is adjusted for the new securities by a set of augmented connections, which are optimized using the new data. The auxiliary connections are constrained to be of low rank. This not only allows us to rapidly optimize for the new task but also reduces the storage and run-time complexity during the deployment phase. The efficiency of our approach is empirically validated in the stock mid-price movement prediction problem using a large-scale limit order book dataset. Experimental results show that our approach enhances prediction performance as well as reduces the overall number of network parameters.

==> old_comments.tex <==

\clearpage
\section{ANSWERS TO REVIEWERS COMMENTS}
This paper was previously submitted to the journal with a paper ID "NEUNET-D-21-00404". We addressed all Reviewers' comments and we  also provide a point-to-point response for each of the comments. 
\\
\\
\\
\\
\textbf{Reviewer \#1}
\\
\\
\textbf{Comment \#1}
\\
\textit{Although the author claimed the proposed method could be easily generalized to other architectures, the effect of the method is unknown when applied to different architectures. It will be more convincing if there are more comparative experiments.}
\\
\\
\textbf{Reply}
\\
We would like to thank the Reviewer for this comment. In this paper, we propose an efficient approach to tackle the transfer learning/domain adaptation problems that are often seen in financial time-series analysis. The proposed approach was demonstrated for the Temporal Attention augmented Bilinear Layer (TABL) network, which is a state-of-the-art architecture for the mid-price direction prediction problem. The same idea can be adapted for other architectures, such as Convolutional Neural Networks (CNNs). In the revised manuscript, we have provided additional experimental results for CNNs in Section 5. The results suggest that our idea can indeed generalize to CNNs. 
\\
\\
\textbf{Comment \#2}
\\
\textit{The old and new datasets in the experiments are divided by stocks, following the title ``incremental multi-stock" and the definition of the research problem. However, generally in practice, the amount of stocks is relatively stable while the daily price data are generated every trading day. I concern whether the method will still work while the old and new datasets are divided by time.}
\\
\\
\textbf{Reply}
\\
While we agree with the Reviewer that the number of stocks does not change dramatically, the number of new Publicly Traded Companies that are listed on the exchanges is not small. Please see, for example, the IPO calendar of Nasdaq (https://www.nasdaq.com/market-activity/ipos). Moreover, the practical aspect of the incremental multi-stock scenario comes when a trader has a portfolio which includes a number of stocks (a subset of all available stocks) and at some point of time he/she includes one/few more.
\\
\\
As the Reviewer pointed out, our proposed method is also applicable for the online learning scenario in which the model needs to adapt to the new data of the same stock. We have run additional experiments for this learning scenario, which is called forward validation experiment setup in Section 5.4. More specifically, we define the following forward validation experimental protocol:

\begin{itemize}
    \item The baseline model is trained for all stocks using the data coming from the first five days.
    \item The standard finetune model is produced by taking the \texttt{baseline} model and finetuning with the data from the 6th and 7th days. 
    \item The augmented model is produced by taking the baseline model and adapting it using the proposed method with the data from the 6th and 7th days. 
    \item All models are evaluated with the data from the 8th, 9th and 10th days. 
\end{itemize}


\noindent The results for this experimental setup demonstrate that our proposed model adaptation approach can provide better results than the standard finetuning approach in this scenario too. 
\\
\textbf{Comment \#3}
\\
\textit{From Table 1, it is not obvious that the performances of TABL-finetune models are lower than the ones of TABL-base.}
\\
\\
\textbf{Reply}
\\
We would like to thank the Reviewer for pointing out this issue. We have now updated the experimental results (by following the suggestions of the Reviewer to also add another type of model), and we have updated the text as follows:
\\
\\
\textit{From the experimental results in Tables 1 and 2, we can clearly see that on average, the proposed model augmentation approach leads to performance improvements compared to the standard finetuning approach for both TABL and CNN network architectures. In addition, by adapting the pretrained models on the new data using the proposed augmentation approach, we indeed observed performance improvements compared to the scenario when the pretrained models are not adapted to the new data, i.e., \texttt{TABL-base} and \texttt{CNN-base}. This was not always the case for the standard finetuning approach since we observed performance degradation when comparing the performance of \texttt{CNN-finetune} and \texttt{CNN-base}. Regarding the two implementation strategies conducted for the TABL architectures, we can see that both strategies lead to very similar results. The differences stem from the stochastic nature of the optimizer as well as the initialization of the network parameters. Here we should note again that after the training process, the models obtained by our method have the same computational and memory complexities as the baseline or finetuned models.}
\\
\\
\\
\\
\textbf{Comment \#4}
\\
\textit{The experiment setup 2 and the result in Table 2 are not fine-grained enough to validate the assumption that the model with the proposed method will work well on both old and new datasets.}
\\
\\
\textbf{Reply}
\\
In experiment setup 2, we do not predict the stock data related to $\mathcal{D}_{\textrm{old}}$ by using the new model $\mathcal{N}_{\textrm{new}}$. The question that this experiment is designed to answer is whether, given $\mathcal{N}_{\textrm{old}}$ and $\mathcal{D}_{\textrm{old}}$, we can build a new model $\mathcal{N}_{\textrm{new}}$ to work well on $\mathcal{D}_{\textrm{new}}$. That is, we do not aim to have a single model that works well for both old and new stocks, but to take advantage of the model that was built for the old stocks to learn a new model for the new stock. Here we should also note that in real-life scenarios, it is desirable to have stock-specific models (and some times time period-specific models). 
\\
\\
\\
\\
\textbf{Comment \#5}
\\
\textit{The author states the maximum rank value is chosen through validation, but no actual analysis is presented. It's not clear how the different low-rank value influences the result.}
\\
\\
\textbf{Reply}
\\
We followed the Reviewer’s suggestion and added in the revised paper the experiment results for different values of the rank (1 to 20). The results for both implementation strategies are shown in Figure 3 and Figure 4 in the revised manuscript (which are shown here as Figure \ref{fig:ranked_IS1} and Figure \ref{fig:ranked_IS2}). The following observation is also added to the revised manuscript:

\begin{figure*}[h]
\centering
        \includegraphics[width=0.9\textwidth]{figs/IS1.eps}%
        \caption{Performance of \texttt{\textbf{aTABL-IS1}} using different rank values }
        \label{fig:ranked_IS1}
\end{figure*}
\begin{figure*}[h]
\centering
        \includegraphics[width=0.9\textwidth]{figs/IS2.eps}%
        \caption{Performance of \texttt{\textbf{aTABL-IS2}} using different rank values}
        \label{fig:ranked_IS2}
\end{figure*}

\textit{The rank value, which is a hyperparameter of the proposed augmentation method, can influence the efficiency in learning complementary knowledge from the new data. As mentioned before in this section, we chose the rank of the augmented models by running experiments on a range of different rank values and selected the one that produces the best F1 score on the training set. Figure 3 and Figure 4 show the effect of different ranks on the test performance of the proposed method. From these figures, it can be seen that there is no clear relation between the rank value and the generalization performance of model. However, we can see that good performance can be obtained from low values of the rank.}
\\
\\
\textbf{Comment \#6}
\\
\textit{There are some mistakes within sentences}\\
\textit{(1) "We want to the information encoded in a encoded in a ..."}\\
\textit{(2) "We denote models following tis TL approach as TABL-finetune."}\\
\textit{(3) "...we finetune a new textttTABL-base using its training data..."}
\\
\\
\textbf{Reply}
\\
We have followed the Reviewer’s suggestions and corrected these typos and grammatical issues.
\\
\\
\\ 
\\ 
\noindent\makebox[\linewidth]{\rule{\paperwidth}{0.4pt}}
\\
\\
\\
\textbf{Reviewer \#2}
\\
\\
\textbf{Comment \#1}
\\
\textit{Dear Authors, the paper with a title Augmented Bilinear Network for Incremental Multi-Stock Time-Series Classification is good writen with a lot of new results and approaches. The paper could very significantly contribute into this field of research. I only recommend extended discussion part in manuscript and compare approach presented in paper with some new recently published approaches for example as :} 
\\
\textit{1- Support spinor machine(2017) Digital Signal Processing: A Review Journal, 70, pp. 59-72,}
\\
\textit{2- The study of Thai stock market across the 2008 financial crisis(2016) Physica A: Statistical Mechanics and its Applications, 462, pp. 117-133. }
\\
\textit{After these mirror corrections paper should be accepted for publication in your journal.}
\\
\\
\textbf{Reply}\\
We would like to thank the Reviewer for his/her positive view of our paper and the suggestions. We have revised our manuscript and added the suggested references.
\\
\\ 
\\ 
\noindent\makebox[\linewidth]{\rule{\paperwidth}{0.4pt}}
\\
\\
\\
\textbf{Reviewer \#3}
\\
\\
\textbf{Comment \#1}
\\
\textit{
I think the objective and application scenario are a little confused and needs more details to clarify. As we know, the financial market is so important that most institution investors would use resources as possible as they can to get the best model. So why we need to use pre-trained model for other stocks especially when new data are available instead of training a brand-new model? How the performance was impacted with/without pretrained model?
}
\\
\\
\textbf{Reply}
\\
We agree with the Reviewer that in the ideal scenario, the more data one can use to optimize his/her model, the better the generalization performance can be. However, in practice, optimizing a model from scratch can be very costly and significantly affects the profitability in the application under consideration in this paper. In addition, there could be the scenario when the pretrained model was purchased through a third-party provider but we do not have access to the proprietary data that it was trained on. 
\\
\\
\\
\textbf{Comment \#2}
\\
\textit{For financial market, only discussion of the statistic metrics seems not that meaningful, since the final goal is to maximize the return. For example, for stock 1, all metrics are around 65\%, how this numbers impact the return and how the predicted price compared with actual price intuitively? I suggest authors draw some figures to show the comparison between the above values so that readers can have a direct evaluation of the model performance.
}
\\
\\
\textbf{Reply}
\\
The mid-price is a quantity that can reflect the dynamics of the order book, thus the dynamics of the supply and demand of the underlying asset. The mid-price is a virtual quantity in the sense that no trade can happen at that price since it is calculated as the middle point between the best bid and best ask prices. Even though the future movements of the mid-price can help the analyst to assess the supply and demand in the market, making profits with such information depends on the particular trading strategy, which is out of scope of this paper.

Here we should also note that the performance metrics used in our experiments are the one used by most of the recently published machine learning papers using this data, in order to evaluate the performance of their methods.
\\
\\
\textbf{Comment \#3}
\\
\textit{The authors only compared with methods that TABL based. But I'm more interested to see how the model performance compared with other state-of-the-art time series prediction models, as even though the proposed model performed the best here, if no advantages when compared with other time series models, then the applications will be much limited.
\\
}
\\
\\
\textbf{Reply}
\\
We have followed the Reviewer’s suggestions and added the experiment results for Convolutional Neural Network (CNN) in the Experiment Section.  
